An Empirical Analysis of Compatibility Issues for Industrial Mobile Games

Detecting and fixing compatibility issues is critical for mobile game development. The rapid evolution of mobile operating systems and device fragmentation make it challenging for developers to timely address these issues across diverse models. Undetected compatibility problems can severely impact user experience and cause financial loss to companies and players. However, mobile game testing remains highly challenging, and compatibility issues are largely underexplored by the research community. To bridge this gap, we conduct an empirical study on common compatibility issues in commercial mobile games. We select four active and representative games with well-documented bug reports, totaling over seven million lines of code and over 20,000 commits. We build a comprehensive dataset linking bugs and fixes, enabling investigation into prevalent symptoms, root causes, and fixing strategies. Through extensive manual analysis, we categorize the most common symptoms and root causes, and summarize the typical fixes for each category. Our findings provide practical guidance for developers and offer insights to inspire future research on testing and fixing compatibility issues in mobile games.

==> summary.tex <==
\begin{table*}[hbpt]
\centering
\caption{Summary of findings and implications about compatibility issues }
\label{tab:summary}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|l|l@{}}
\toprule
\# &
  \textbf{Findings about compatibility issues Symptoms} &
  \textbf{Implications} \\ \midrule
1 &
  \begin{tabular}[c]{@{}l@{}}The top three symptoms of compatibility issues is UI Exception, \\ Installation or Startup Failure and Crash.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Techniques for detecting compatibility issues should focus\\  on these three types of symptoms.\end{tabular} \\ \hline
2 &
  \begin{tabular}[c]{@{}l@{}}Most issues (80\%) appear as UI Exception. In most cases the game \\ can continue running even if these issues occur. UI Layout issues take \\ up  55\% of all compatibility issues, and 69\% inside UI Exception issues.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}UI exception is the core direction to develop techniques\\ for automatically detecting compatibility issues. Since these \\ issues won't kill game process, the feasible way to detect them\\  is CV techniques.\end{tabular} \\ \hline
3 &
  \begin{tabular}[c]{@{}l@{}}Compared with the Crashes (5.5\%), Installation or Startup Failure \\ (11\%) occurs more frequently.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Compared to the crashes, developers should pay more attention\\ to the game installation and startup.\end{tabular} \\ \midrule
 &
  \textbf{Findings about compatibility issues Root Causes} &
  \textbf{Implications} \\ \midrule
4 &
  \begin{tabular}[c]{@{}l@{}}The top three root causes of compatibility issues is Display Adaption, \\ Computation Unit Performance and System/SDK Version.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Techniques for fixing compatibility issues should focus on these \\ three types.\end{tabular} \\ \hline
5 &
  \begin{tabular}[c]{@{}l@{}}Most issues (55\%) happened as UI Exception because of Display \\ unsuitable on irregular screens.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Developers should pay more attention on the adaptation of \\ irregular-shaped screens from various manufacturers.\end{tabular} \\ \hline
6 &
  Most (80\%) Computation Unit issues are related to GPU performance. &
  \begin{tabular}[c]{@{}l@{}}Developers should consider carefully about the GPU configuration\\ requirements for the games.\end{tabular} \\ \midrule
 &
  \textbf{Findings about compatibility issues Fixing Strategies} &
  \textbf{Implications} \\ \midrule
7 &
  \begin{tabular}[c]{@{}l@{}}Most Irregular-shaped Screen issues (70\%) are fixed by partially adjust \\ UI layout near notch.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}During the developing process of mobile games, UI layout should\\ be personalized for the screen shape of popular devices.\end{tabular} \\ \hline
8 &
  \begin{tabular}[c]{@{}l@{}}Most Background Image Resolution issues (88\%) are fixed by modifying\\ the size and resolution of images.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Developers should prepare the background images for multiple \\ resolutions in advance to make sure the appearance correct.\end{tabular} \\ \hline
9 &
  \begin{tabular}[c]{@{}l@{}}Computation Unit Performance issues are usually fixed by customizing\\ low-configuration settings, such as reducing the quality of shaders and\\ resources, or disabling rendering techniques.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Building multiple configuration options in the game is an effective \\ way to avoid performance issues.\end{tabular} \\ \hline
10 &
  \begin{tabular}[c]{@{}l@{}}For installation Failure issues, adding 32-bit system support is a feasible \\ way, but it will also increase the size of the game package.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}32-bit system support should be added with pertinence. Adding into\\  the general installation package is not a good choice.\end{tabular} \\ \bottomrule
\end{tabular}
}
\end{table*}
